Robust Shape Estimation for 3D Deformable Object Manipulation

Existing shape estimation methods for deformable object manipulation suffer from the drawbacks of being off-line, model dependent, noise-sensitive or occlusion-sensitive, and thus are not appropriate for manipulation tasks requiring high precision. In this paper, we present a real-time shape estimation approach for autonomous robotic manipulation of 3D deformable objects. Our method fulfills all the requirements necessary for the high-quality deformable object manipulation in terms of being real-time, model-free and robust to noise and occlusion. These advantages are accomplished using a joint tracking and reconstruction framework, in which we track the object deformation by aligning a reference shape model with the stream input from the RGB-D camera, and simultaneously upgrade the reference shape model according to the newly captured RGB-D data. We have evaluated the quality and robustness of our real-time shape estimation pipeline on a set of deformable manipulation tasks implemented on physical robots. Videos are available at https://lifeisfantastic.github.io/DeformShapeEst/

==> sec_2.tex <==
\section{Related Work}
\label{sec:related_work}
The complex behavior of deformable objects brings a challenge in its perception and manipulation. Due to this reason, many existing methods prefer employing predefined models to approximate the soft objects for specific tasks. For example, a polygonal model is proposed in~\cite{doumanoglou2016folding} to solve the cloth type and shape recognition problem for robotic garments folding. Furthermore, to generate more accurate and refined shape estimation for highly deformable objects, one sophisticated solution is to conduct physically-based simulation based on the Finite Element Method (FEM). Such FEM-based simulation is widely used to deal with challenging problems like tissue state estimation in robot-assisted surgery ~\cite{patil2010toward, sinha2014modeling} and cloth simulation in robot-assisted dressing ~\cite{erickson2017does}. Recent progress in visual perception, especially the development of commercial RGB-D cameras, provides a new opportunity for solving the real-world deformable object manipulation problem rather than pure simulation. In~\cite{schulman2013tracking}, a probabilistic observation model is presented to determine the correspondence between the live depth measurement and a virtual mass-spring model. The correspondence is then used to drive the physically-based simulator for the shape tracking of deformable objects like ropes. \cite{loper2015smpl,joo2018total} aligned 3D point clouds with generative deformation model to capture the movements of principal human parts like body or even face and hands.

One common limitation of the above methods is that they strongly depend on the prior knowledge of both the shape model and deformation model, which arises difficulty when extending them to deal with more general deformable objects. \cite{li2014real,zollhofer2014real} partially solve this problem by decreasing the reliance on a predefined deformation model. They divide the shape estimation problem into two phases, including an offline reconstruction step and an online tracking step. In their reconstruction step, they keep a deformable object stationary and scan it using one RGB-D camera. Then they accumulate all the captured depth images into a full surface model using KinectFusion~\cite{newcombe2011kinectfusion}. In the tracking step, the object is deforming, and the live depth image from a streaming camera is aligned with the reconstructed surface model to estimate the object's live shape. One main difference between these two methods is that~\cite{li2014real} does not consider the object's deformation behavior and requires numerous shape-varying reconstruction as a database for online tracking; while~\cite{zollhofer2014real} improves the pipeline by approximating the deformation of general soft objects with the as-rigid-as-possible (ARAP) constraint~\cite{sorkine2007rigid}, which enables the method to start up with only a single offline surface reconstruction.
Note that the offline reconstruction step in these two methods still rely on the assumption of stationary objects, which may bring inconvenience in practical applications. Recently, DynamicFusion~\cite{newcombe2015dynamicfusion} makes the first attempt to embed the tracking and reconstruction steps into a unified online framework and provides compelling results. This method updates both the shape model and the deformation model iteratively and is independent of the prior knowledge of the target object.

Another branch of work is the shape seroving~\cite{navarro2016automatic,navarro2018fourier,hu20173d,jia2017manipulating}, which aim at providing the real-time and model-free solution for the deformable object perception and control. Instead of employing full image data for shape modeling and estimation, these methods share the similar idea with the visual servoing by extracting partial but important features from the input image to approximate the shape state. Because the shape feedback defined in the feature space is usually low-dimensional, current shape servoing methods can learn a mapping function between the feature state and the control signal directly through the online learning algorithm. Such online control policy learning framework contributes to their advantages of being real-time and model-free. Note that the selected features in shape servoing must be highly related to the accomplishment of the task, and thus one critical issue in this technique is to propose an appropriate feature descriptor that can achieve efficient control policy learning. Early work in this line~\cite{navarro2016automatic,hu20173d} use manually designed features responsive to local surface patterns like as points, normals or curvatures. High-level geometry features, such as truncated Fourier series~\cite{navarro2018fourier} and the histogram of oriented wrinkles (HOW)~\cite{jia2017manipulating} are also proposed in follow-up work for better shape representation.

